Spoken Moments: Learning Joint Audio-Visual Representations from Video Descriptions

When people observe events, they are able to abstract key information and build concise summaries of what is happening. These summaries include contextual and semantic information describing the important high-level details (what, where, who and how) of the observed event and exclude background information that is deemed unimportant to the observer. With this in mind, the descriptions people generate for videos of different dynamic events can greatly improve our understanding of the key information of interest in each video. These descriptions can be captured in captions that provide expanded attributes for video labeling (e.g. actions/objects/scenes/sentiment/etc.) while allowing us to gain new insight into what people find important or necessary to summarize specific events. Existing caption datasets for video understanding are either small in scale or restricted to a specific domain. To address this, we present the Spoken Moments (S-MiT) dataset of 500k spoken captions each attributed to a unique short video depicting a broad range of different events. We collect our descriptions using audio recordings to ensure that they remain as natural and concise as possible while allowing us to scale the size of a large classification dataset. In order to utilize our proposed dataset, we present a novel Adaptive Mean Margin (AMM) approach to contrastive learning and evaluate our models on video/caption retrieval on multiple datasets. We show that our AMM approach consistently improves our results and that models trained on our Spoken Moments dataset generalize better than those trained on other video-caption datasets.

==> section/5_result_caption_generation.tex <==
\subsection{Caption Generation}
To further examine the strength of the representations, we learn with the Spoken Moments dataset to the task of caption generation using the encoder-decoder transformer architecture~\cite{transformer2017neurips,dense2018cvpr}. Specifically, we extract feature vectors from the representation layer before the projection layer of our video model and use them as input to the encoder.
We use the Transformer with the hidden unit size of 2048, two layers, 8 heads, and the dropout of 0.2. We train models with a learning rate of 0.1 with a linear decay schedule. We evenly sample two frames per second from each video and set the maximum sentence length as 20.
In order to emphasize the difference between the different datasets, we keep the settings all the same for the baseline models we train. 

We compare the results of transferring the representations learned using the different loss functions (SHN, NCE, MMS, AMM) described in Section~\ref{sec:approach} for generating captions for the videos of the Spoken Moments and the Vatex-en dataset~\cite{Wang_2019_ICCV}.
We additionally train caption models on the Vatex-en dataset to use as baselines on the dataset as an example of the difficulty in cross dataset generalization for video captioning datasets.  
In Table \ref{table:caption_cross_evaluation}, we report the caption generation results on the Vatex-en and Spoken Moments datasets using the commonly used BLEU@\{3,4\} \cite{bleu2002acl} and METEOR \cite{methor2005acl} metrics (i.e. higher numbers are better).
It is shown that all the Spoken Moments models generalize well to the Vatex-en dataset, while the Vatex-en models fail to generate accurate descriptions on Spoken Moments. This is expected due to the difference in scale and diversity of the two datasets (Table~\ref{table:data_comparison}).
In Figure~\ref{fig:caption_generation_spoken}, we show some caption generation examples on the videos from the Spoken Moments dataset. It is observed that our Spoken Moments model uses a larger vocabulary and can describe videos better with more accurate descriptions.

The models trained with the different loss functions all perform similarly in the task with the SHN model achieving slightly better results. This performance similarity is likely due to all of the models initially being trained to align to pretrained BART representations. The edge of SHN here is possibly attributed to the fact that it is trained to increase the discrepancy from similar examples, improving discriminative feature generation, while the other loss functions directly optimize general retrieval. 


\begin{table}[h]
\centering
\scalebox{0.75}{
    \centering
    \begin{tabular}{c | c | c  c  c | c  c  c  }
        \Xhline{0.8pt}
        %\multirow{3}{*}{} & \multicolumn{6}{c}{\textbf{Test Dataset}} \\ \cline{2-7}
        Training & Loss & \multicolumn{3}{c|}{Vatex-en}  & \multicolumn{3}{c}{Spoken Moments} \\
        \cline{3-8}
        Dataset & Function & B@3 & B@4 & M & B@3 & B@4 & M \\
        \Xhline{0.8pt}
        \multirow{4}{*}{Vatex-en}
            & SHN & \textcolor{blue}{\textbf{6.407}} & 2.326 & 10.368 & \textbf{1.804} & \textbf{0.554} & \textbf{7.791} \\
            & NCE & 6.274 & 2.245 & 10.299 & 1.723 & 0.515 & 7.751 \\
            & MMS & 6.406 & \textcolor{blue}{\textbf{2.349}} & \textcolor{blue}{\textbf{10.373}} & 1.686 & 0.503 & 7.684 \\
            & AMM & 6.298 & 2.222 & 10.257 & 1.743 & 0.473 & 7.693 \\
        \hline
        \multirow{4}{*}{S-MiT} 
            & SHN & 5.555 & 1.898 & \textbf{9.807}& \textcolor{blue}{\textbf{3.169}} & 1.185 & \textcolor{blue}{\textbf{9.571}} \\
            & NCE & \textbf{5.574} & 1.890 & 9.700 & 3.077 & 1.146 & 9.422 \\
            & MMS & 5.563 & \textbf{1.948} & 9.784 & 3.037 & 1.154 & 9.394 \\
            & AMM & 5.461 & 1.865 & 9.646 & 3.161 & \textcolor{blue}{\textbf{1.257}} & 9.479 \\
        \Xhline{0.8pt}
    \end{tabular}}
\caption{\textbf{Cross Evaluation of Caption Generation Performance:} 
We compare the results of fine-tuning our video models trained with different loss functions on video caption generation.  We train the models to generate captions for the Spoken Moments dataset (S-MiT) and evaluate them on caption generation for S-MiT and Vatex-en.  We include models trained on the Vatex-en dataset as baselines to show how well our models can generalize to another dataset.  We evaluate our models on the commonly used BLEU (B) and METEOR (M) metrics. Bold numbers indicate the best performance among the models trained on the same dataset while we color the best scores across different datasets in blue.}
\label{table:caption_cross_evaluation}
\end{table}

\begin{figure*}[h]
    \centering
	\begin{tabularx}{\textwidth}{ p{1.3cm} | X X X}
	    %& \includegraphics[width=0.27\textwidth, trim={1.5cm 0 1.5cm 0},clip]{figures/caption_generation/spoken/1.jpg}
	    & \includegraphics[width=0.27\textwidth]{figures/caption_generation/spoken/1.jpg}
	    & \includegraphics[width=0.27\textwidth]{figures/caption_generation/spoken/2.jpg} 
	    & \includegraphics[width=0.27\textwidth]{figures/caption_generation/spoken/3.jpg}
	    \\
	    
	    \tiny{GT} 
	    & \tiny{sprinkler rotates watering the lawn}
	    & \tiny{people screaming and cheering in the street as they send what pink balloons up in the air}
	    & \tiny{it's a club there are people dancing and there's red and blue lights flashing}
	    \\
	    
	    \cellcolor{yellow!20} \tiny{S-MiT} 
	    & \cellcolor{yellow!20} \tiny{a \textbf{sprinkler} is watering the grass}
	    & \cellcolor{yellow!20} \tiny{a large crowd of people are gathered in a \textbf{protest}}
	    & \cellcolor{yellow!20} \tiny{a concert is going on with \textbf{lights flashing}}
	    \\
	    
	    \cellcolor{green!10} \tiny{Vatex-en}
	    & \cellcolor{green!10} \tiny{a man is using a hose to water the plants in a garden}
	    & \cellcolor{green!10} \tiny{a group of people are standing around a table and talking}
	    & \cellcolor{green!10} \tiny{a man is playing a guitar while another man is playing a guitar}
    \end{tabularx} 
	\hline
    
\caption{Caption generation examples on Spoken Moments. Compared to the model trained on Vatex-en (Vatex-en), the model trained on Spoken Moments (S-MiT) generates captions with broader vocabulary.}    
\label{fig:caption_generation_spoken}
\end{figure*} 

==> section/B_old_caption_datasets.tex <==
\section{Caption Datasets}

There have been a number of different datasets released for providing language descriptions of visual information.  For images, Flickr8k \cite{Hodosh2013FramingID} and Flickr30k \cite{Plummer_2015_ICCV} include 8k and 30k images respectively each sourced from Flickr.  Each image is associated with 5 text captions describing what is in the image.  An additional set of 5 audio captions per image in both sets was also recently collected for learning joint embeddings between speech and images \cite{david2020ijcv}.  The Visual Genome dataset \cite{krishnavisualgenome} includes separate captions for multiple regions of more than 180k images allowing for fine-grained descriptions of each image.  The Places Audio Caption dataset \cite{NIPS2016_6186} contains approximately 400k images from the Places 205 \cite{NIPS2014_5349} image dataset with audio captions of people verbally describing each image. MS COCO \cite{capeval2015} is a large image dataset for object recognition, segmentation, and captioning which includes roughly 1 million captions for 160k images sourced from Flickr.  Conceptual Captions \cite{sharma2018conceptual} contains 3.3M images with captions generated from HTML attributes associated with web based images. The Stock3M dataset \cite{Wang_2017_CVPR} includes 3.2 million images each with a crowdsourced caption.

Beyond the numerous datasets available or image captioning \cite{Hodosh2013FramingID,Plummer_2015_ICCV,krishnavisualgenome,capeval2015,sharma2018conceptual,Wang_2017_CVPR}, including those that provide spoken descriptions \cite{NIPS2016_6186,david2020ijcv}, there are a variety of different video caption datasets available. A number of these datasets are related to cooking \cite{tacos:regnerietal:tacl,cispa1826,10.1007/s11263-015-0851-8} including YouCook \cite{DaXuDoCVPR2013} and YouCook II \cite{Zhou2018TowardsAL} which includes 2k videos from YouTube each with multiple captions annotated at different segments of each video. MPII-Movie Description Corpus \cite{7298940} contains transcribed audio descriptions from 94 Hollywood movies split into 68k clips %with an average length of 3.9 seconds 
where each clip is paired with a sentence from the movies script and an audio description of the visual content in each clip.  %M-VAD \cite{} contains 49k video clips sourced from 92 movies with an average length of 6.2 seconds per clip where each clip is paired with a short text description.  
VideoStory \cite{gella-etal-2018-dataset} contains 20k social media videos where each video contains a paragraph length description. The ActivityNet Captions dataset \cite{krishna2017dense} has 20k videos with 100k text descriptions.% with an average of 13.48 words per description and pertains to an average clip length of 36 seconds.  
The Microsoft Video Description (MSVD) dataset \cite{chen-dolan-2011-collecting} contains 2k YouTube clips with a 10-25 second duration and an average of 41 single sentence descriptions per clip.  
MSR-Video to Text (MSR-VTT) \cite{xu2016msr-vtt} contains 7k videos split into 10k clips with 20 captions per video. % for a total of 200k captions.
HowTo100M \cite{miech19howto100m} contains 136 million clips sourced from 1.22 million instructional videos with narrations generated from subtitles associated for each video.  While HowTo100M is the largest of these video caption datasets, the captions are not human verified and the content is constrained to instructional videos.  VaTeX \cite{Wang_2019_ICCV} contains 41k videos sourced from the Kinetics-600 dataset \cite{DBLP:journals/corr/KayCSZHVVGBNSZ17,carreira2018short} annotated with 10 English captions and 10 Chinese captions for multilingual captioning.  VaTeX is the most similar to our proposed dataset in that it is sourced from an existing video dataset for action recognition and the captions are directly annotated. %While we do not provide 10 English captions per video, here 
We \textbf{vastly expand on the scale of these datasets and record spoken captions for 500k unique three second clips} each with different source videos from the Moments in Time dataset \cite{monfortmoments,monfort2019multimoments}.

==> section/D_retrieval_task.tex <==
\begin{table*}[tb]
    \scalebox{0.62}{
    \begin{tabular}{ c | c | c  c  c  c | c  c  c  c | c  c  c  c }
        \Xhline{0.8pt}
        \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Loss}} & \multicolumn{4}{c|}{\textbf{Caption to Video}} & \multicolumn{4}{c|}{\textbf{Video to Caption}} & \multicolumn{4}{c}{\textbf{Mean}} \\
         & & R@1 & R@5 & R@10 & mAP & R@1 & R@5 & R@10 & mAP & R@1 & R@5 & R@10 & mAP \\
        \Xhline{0.8pt}
        \multirow{5}{*}{Vatex \cite{Wang_2019_ICCV}}
        & NCE & 43.6\std{1.4} & 77.4\std{1.4} & 86.5\std{1.4} & 58.4\std{1.2} & 39.4\std{1.3} & 74.3\std{1.0} & 84.7\std{0.8} & 54.7\std{1.0} & 41.5\std{1.2} & 75.8\std{1.1} & 85.6\std{1.1} & 56.5\std{1.0}\\
        & SHN & 19.6\std{1.4} & 50.2\std{1.5} & 63.9\std{0.6} & 33.8\std{1.1} & 22.9\std{1.0} & 54.0\std{0.9} & 68.8\std{1.2} & 37.6\std{0.9} & 21.3\std{0.9} & 52.1\std{0.8} & 66.3\std{0.8} & 35.7\std{0.7}\\
        & MMS & 46.2\std{1.5} & 79.7\std{0.8} & 88.1\std{0.8} & 60.7\std{1.0} & 42.0\std{0.7} & 77.7\std{0.7} & \textbf{86.8}\std{0.3} & 57.5\std{0.6} & 44.1\std{1.1} & 78.7\std{0.7} & 87.4\std{0.5} & 59.1\std{0.7}\\
        & AMM & \textbf{48.7}\std{1.4} & \textbf{82.0}\std{0.9} & \textbf{89.3}\std{1.1} & \textbf{63.0}\std{1.0} & \textbf{43.0}\std{0.7} & \textbf{77.4}\std{1.1} & \textbf{85.8}\std{0.7} & \textbf{58.3}\std{0.6} & \textbf{45.9}\std{1.0} & \textbf{79.7}\std{0.4} & \textbf{87.5}\std{0.8} & \textbf{60.7}\std{0.6}\\
        \hline
        \multirow{5}{*}{ActivityNet \cite{krishna2017dense}}
        & NCE & 11.8\std{0.6} & 35.4\std{1.0} & 50.6\std{0.8} & 23.8\std{0.4} & 16.7\std{0.8} & 43.0\std{1.2} & 57.1\std{1.2} & 29.5\std{0.8} & 14.3\std{0.6} & 39.2\std{0.8} & 53.8\std{1.0} & 26.7\std{0.5}\\
        & SHN & 9.9\std{0.9} & 31.2\std{1.3} & 45.2\std{0.9} & 20.9\std{0.9} & 13.7\std{1.1} & 38.5\std{0.9} & 53.4\std{0.9} & 25.9\std{1.0} & 11.8\std{0.9} & 34.9\std{0.8} & 49.3\std{0.7} & 23.4\std{0.9}\\
        & MMS & 12.0\std{0.7} & 35.5\std{1.0} & 49.2\std{0.8} & 23.9\std{0.6} & 16.2\std{0.4} & 42.4\std{0.9} & 56.5\std{1.6} & 28.8\std{0.6} & 14.1\std{0.4} & 39.0\std{0.2} & 52.8\std{1.2} & 26.4\std{0.2}\\
        & AMM & \textbf{17.2}\std{1.1} & \textbf{46.1}\std{1.4} & \textbf{60.0}\std{0.8} & \textbf{30.6}\std{0.6} & \textbf{20.9}\std{1.1} & \textbf{50.1}\std{1.3} & \textbf{62.4}\std{0.8} & \textbf{34.3}\std{0.6} & \textbf{19.1}\std{1.0} & \textbf{48.1}\std{1.2} & \textbf{61.2}\std{0.6} & \textbf{32.5}\std{0.6}\\
        \hline
        \multirow{5}{*}{MSR-VTT \cite{xu2016msr-vtt}}
        & NCE & 20.7\std{0.9} & 51.0\std{0.7} & 66.6\std{1.2} & 35.0\std{0.4} & 30.7\std{1.4} & 65.1\std{0.7} & 78.2\std{1.3} & 46.1\std{1.2} & 25.7\std{1.0} & 58.1\std{0.6} & 72.4\std{1.2} & 40.6\std{0.7}\\
        & SHN & 11.3\std{0.2} & 32.0\std{1.0} & 44.9\std{1.4} & 21.9\std{0.3} & 22.1\std{0.9} & 54.5\std{1.6} & 68.9\std{1.4} & 37.0\std{1.1} & 16.7\std{0.5} & 43.3\std{0.5} & 56.9\std{0.9} & 29.5\std{0.5}\\
        & MMS & 17.6\std{1.1} & 46.5\std{0.9} & 61.6\std{0.9} & 31.5\std{0.6} & \textbf{28.3}\std{1.1} & \textbf{63.1}\std{1.4} & \textbf{76.1}\std{0.9} & \textbf{43.8}\std{1.1} & 23.0\std{0.9} & 54.8\std{0.6} & 68.9\std{0.7} & 37.6\std{0.6}\\
        & AMM & \textbf{25.7}\std{0.8} & \textbf{61.0}\std{0.8} & \textbf{75.6}\std{0.7} & \textbf{41.6}\std{0.6} & \textbf{32.5}\std{1.5} & \textbf{67.5}\std{1.7} & \textbf{80.1}\std{1.4} & \textbf{48.0}\std{1.2} & \textbf{29.1}\std{0.8} & \textbf{64.2}\std{1.0} & \textbf{77.9}\std{1.0} & \textbf{44.8}\std{0.8}\\
        \hline
        \multirow{5}{*}{S-MiT}
        & NCE & 28.7\std{2.1} & 60.9\std{1.1} & \textbf{73.7}\std{1.1} & 43.4\std{1.7} & 37.5\std{1.5} & 67.0\std{1.4} & 77.0\std{1.0} & 50.9\std{1.2} & 33.1\std{1.8} & 64.0\std{1.2} & \textbf{75.3}\std{1.0} & 47.2\std{1.5}\\
        & SHN & 23.0\std{1.3} & 54.2\std{2.7} & 67.7\std{1.3} & 37.5\std{1.5} & 36.2\std{1.2} & 64.9\std{1.8} & 76.1\std{0.8} & 49.3\std{1.0} & 29.6\std{1.2} & 59.6\std{2.1} & 71.9\std{1.0} & 43.4\std{1.2}\\
        & MMS & 28.8\std{2.1} & 60.5\std{1.7} & 73.5\std{0.9} & 43.4\std{1.8} & 38.5\std{1.5} & 66.9\std{1.4} & 76.8\std{1.5} & 51.4\std{1.4} & 33.7\std{1.7} & 63.7\std{1.5} & 75.1\std{0.9} & 47.4\std{1.6}\\
        & AMM & \textbf{30.5}\std{1.9} & \textbf{61.4}\std{1.8} & 73.1\std{1.3} & \textbf{44.7}\std{1.7} & \textbf{39.1}\std{2.1} & \textbf{67.4}\std{1.9} & \textbf{77.2}\std{1.6} & \textbf{51.9}\std{1.9} & \textbf{34.8}\std{1.9} & \textbf{64.4}\std{1.8} & 75.1\std{1.4} & \textbf{48.3}\std{1.7}\\
        \Xhline{0.8pt}
    \end{tabular}}
\caption{\textbf{Loss Function Comparison for Video/Caption Retrieval:}  Models trained on four datasets with different loss functions are compared for video/caption retrieval.  Results are averaged over five random sets of 1k video-caption pairs from the test set for each dataset.  The proposed AMM loss function consistently achieves the best performance.}
\label{table:loss_comparison}
\end{table*}

\section{Video/Caption Retrieval}

Table~\ref{table:full_loss_comparison_language} shows results on using different combinations of the loss functions and language models on {Vatex}~\cite{Wang_2019_ICCV}, {ActivityNet Captions}~\cite{krishna2017dense}, {MSR-VTT}~\cite{xu2016msr-vtt} as well as the proposed Spoken Moments. 

==> section/D_retrieval_task_old.tex <==
\begin{table*}[tb]
    \scalebox{0.62}{
    \begin{tabular}{ c | c | c  c  c  c | c  c  c  c | c  c  c  c }
        \Xhline{0.8pt}
        \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Loss}} & \multicolumn{4}{c|}{\textbf{Caption to Video}} & \multicolumn{4}{c|}{\textbf{Video to Caption}} & \multicolumn{4}{c}{\textbf{Mean}} \\
         & & R@1 & R@5 & R@10 & mAP & R@1 & R@5 & R@10 & mAP & R@1 & R@5 & R@10 & mAP \\
        \Xhline{0.8pt}
        \multirow{5}{*}{Vatex \cite{Wang_2019_ICCV}}
        & NCE & 43.6\std{1.4} & 77.4\std{1.4} & 86.5\std{1.4} & 58.4\std{1.2} & 39.4\std{1.3} & 74.3\std{1.0} & 84.7\std{0.8} & 54.7\std{1.0} & 41.5\std{1.2} & 75.8\std{1.1} & 85.6\std{1.1} & 56.5\std{1.0}\\
        & SHN & 19.6\std{1.4} & 50.2\std{1.5} & 63.9\std{0.6} & 33.8\std{1.1} & 22.9\std{1.0} & 54.0\std{0.9} & 68.8\std{1.2} & 37.6\std{0.9} & 21.3\std{0.9} & 52.1\std{0.8} & 66.3\std{0.8} & 35.7\std{0.7}\\
        & MMS & 46.2\std{1.5} & 79.7\std{0.8} & 88.1\std{0.8} & 60.7\std{1.0} & 42.0\std{0.7} & 77.7\std{0.7} & \textbf{86.8}\std{0.3} & 57.5\std{0.6} & 44.1\std{1.1} & 78.7\std{0.7} & 87.4\std{0.5} & 59.1\std{0.7}\\
        & AMM & \textbf{48.7}\std{1.4} & \textbf{82.0}\std{0.9} & \textbf{89.3}\std{1.1} & \textbf{63.0}\std{1.0} & \textbf{43.0}\std{0.7} & \textbf{77.4}\std{1.1} & \textbf{85.8}\std{0.7} & \textbf{58.3}\std{0.6} & \textbf{45.9}\std{1.0} & \textbf{79.7}\std{0.4} & \textbf{87.5}\std{0.8} & \textbf{60.7}\std{0.6}\\
        \hline
        \multirow{5}{*}{ActivityNet \cite{krishna2017dense}}
        & NCE & 11.8\std{0.6} & 35.4\std{1.0} & 50.6\std{0.8} & 23.8\std{0.4} & 16.7\std{0.8} & 43.0\std{1.2} & 57.1\std{1.2} & 29.5\std{0.8} & 14.3\std{0.6} & 39.2\std{0.8} & 53.8\std{1.0} & 26.7\std{0.5}\\
        & SHN & 9.9\std{0.9} & 31.2\std{1.3} & 45.2\std{0.9} & 20.9\std{0.9} & 13.7\std{1.1} & 38.5\std{0.9} & 53.4\std{0.9} & 25.9\std{1.0} & 11.8\std{0.9} & 34.9\std{0.8} & 49.3\std{0.7} & 23.4\std{0.9}\\
        & MMS & 12.0\std{0.7} & 35.5\std{1.0} & 49.2\std{0.8} & 23.9\std{0.6} & 16.2\std{0.4} & 42.4\std{0.9} & 56.5\std{1.6} & 28.8\std{0.6} & 14.1\std{0.4} & 39.0\std{0.2} & 52.8\std{1.2} & 26.4\std{0.2}\\
        & AMM & \textbf{17.2}\std{1.1} & \textbf{46.1}\std{1.4} & \textbf{60.0}\std{0.8} & \textbf{30.6}\std{0.6} & \textbf{20.9}\std{1.1} & \textbf{50.1}\std{1.3} & \textbf{62.4}\std{0.8} & \textbf{34.3}\std{0.6} & \textbf{19.1}\std{1.0} & \textbf{48.1}\std{1.2} & \textbf{61.2}\std{0.6} & \textbf{32.5}\std{0.6}\\
        \hline
        \multirow{5}{*}{MSR-VTT \cite{xu2016msr-vtt}}
        & NCE & 20.7\std{0.9} & 51.0\std{0.7} & 66.6\std{1.2} & 35.0\std{0.4} & 30.7\std{1.4} & 65.1\std{0.7} & 78.2\std{1.3} & 46.1\std{1.2} & 25.7\std{1.0} & 58.1\std{0.6} & 72.4\std{1.2} & 40.6\std{0.7}\\
        & SHN & 11.3\std{0.2} & 32.0\std{1.0} & 44.9\std{1.4} & 21.9\std{0.3} & 22.1\std{0.9} & 54.5\std{1.6} & 68.9\std{1.4} & 37.0\std{1.1} & 16.7\std{0.5} & 43.3\std{0.5} & 56.9\std{0.9} & 29.5\std{0.5}\\
        & MMS & 17.6\std{1.1} & 46.5\std{0.9} & 61.6\std{0.9} & 31.5\std{0.6} & \textbf{28.3}\std{1.1} & \textbf{63.1}\std{1.4} & \textbf{76.1}\std{0.9} & \textbf{43.8}\std{1.1} & 23.0\std{0.9} & 54.8\std{0.6} & 68.9\std{0.7} & 37.6\std{0.6}\\
        & AMM & \textbf{25.7}\std{0.8} & \textbf{61.0}\std{0.8} & \textbf{75.6}\std{0.7} & \textbf{41.6}\std{0.6} & \textbf{32.5}\std{1.5} & \textbf{67.5}\std{1.7} & \textbf{80.1}\std{1.4} & \textbf{48.0}\std{1.2} & \textbf{29.1}\std{0.8} & \textbf{64.2}\std{1.0} & \textbf{77.9}\std{1.0} & \textbf{44.8}\std{0.8}\\
        \hline
        \multirow{5}{*}{S-MiT}
        & NCE & 28.7\std{2.1} & 60.9\std{1.1} & \textbf{73.7}\std{1.1} & 43.4\std{1.7} & 37.5\std{1.5} & 67.0\std{1.4} & 77.0\std{1.0} & 50.9\std{1.2} & 33.1\std{1.8} & 64.0\std{1.2} & \textbf{75.3}\std{1.0} & 47.2\std{1.5}\\
        & SHN & 23.0\std{1.3} & 54.2\std{2.7} & 67.7\std{1.3} & 37.5\std{1.5} & 36.2\std{1.2} & 64.9\std{1.8} & 76.1\std{0.8} & 49.3\std{1.0} & 29.6\std{1.2} & 59.6\std{2.1} & 71.9\std{1.0} & 43.4\std{1.2}\\
        & MMS & 28.8\std{2.1} & 60.5\std{1.7} & 73.5\std{0.9} & 43.4\std{1.8} & 38.5\std{1.5} & 66.9\std{1.4} & 76.8\std{1.5} & 51.4\std{1.4} & 33.7\std{1.7} & 63.7\std{1.5} & 75.1\std{0.9} & 47.4\std{1.6}\\
        & AMM & \textbf{30.5}\std{1.9} & \textbf{61.4}\std{1.8} & 73.1\std{1.3} & \textbf{44.7}\std{1.7} & \textbf{39.1}\std{2.1} & \textbf{67.4}\std{1.9} & \textbf{77.2}\std{1.6} & \textbf{51.9}\std{1.9} & \textbf{34.8}\std{1.9} & \textbf{64.4}\std{1.8} & 75.1\std{1.4} & \textbf{48.3}\std{1.7}\\
        \Xhline{0.8pt}
    \end{tabular}}
\caption{\textbf{Loss Function Comparison for Video/Caption Retrieval:}  Models trained on four datasets with different loss functions are compared for video/caption retrieval.  Results are averaged over five random sets of 1k video-caption pairs from the test set for each dataset.  The proposed AMM loss function consistently achieves the best performance.}
\label{table:loss_comparison}
\end{table*}


\begin{table*}[tb]
    \scalebox{0.45}{
    \begin{tabular}{ c | c | c | c  c  c  c | c  c  c  c | c  c  c  c | c  c  c  c  | c  c  c  c }
        \hline
        \multirow{3}{*}{\textbf{Trained On}} & & \multirow{3}{*}{\textbf{Loss}} & \multicolumn{20}{c}{\textbf{Evaluated On}} \\
        \cline{4-23}
        & \textbf{Language} &  & \multicolumn{4}{c|}{\textbf{Vatex}\cite{Wang_2019_ICCV}} & \multicolumn{4}{c|}{\textbf{ActivityNet}\cite{krishna2017dense}} & \multicolumn{4}{c}{\textbf{MSR-VTT}\cite{xu2016msr-vtt}} & \multicolumn{4}{c}{\textbf{S-MiT}} & \multicolumn{4}{c}{\textbf{Mean}} \\
        & \textbf{Model} & & R@1 & R@5 & R@10 & mAP & R@1 & R@5 & R@10 & mAP & R@1 & R@5 & R@10 & mAP & R@1 & R@5 & R@10 & mAP & R@1 & R@5 & R@10 & mAP \\
\hline
\multirow{12}{*}{\textbf{Vatex}} & \multirow{4}{*}{fasttext}
 & NCE & 13.7\std{0.5} & 38.4\std{1.0} & 52.0\std{0.9} & 25.8\std{0.6} & 6.5\std{0.5} & 20.4\std{0.8} & 30.2\std{0.7} & 14.5\std{0.5} & 6.3\std{0.5} & 19.8\std{0.6} & 29.3\std{0.8} & 13.9\std{0.5} & 7.8\std{0.8} & 22.5\std{1.1} & 33.1\std{0.9} & 16.1\std{0.9} & 8.6\std{3.5} & 25.3\std{8.8} & 36.2\std{10.7} & 17.6\std{5.6}\\
 & & SHN & 11.2\std{0.5} & 34.4\std{1.0} & 49.4\std{1.1} & 23.2\std{0.6} & 5.1\std{0.5} & 16.8\std{0.6} & 25.3\std{0.5} & 11.9\std{0.4} & 5.6\std{0.4} & 18.3\std{0.5} & 28.8\std{0.5} & 13.1\std{0.2} & 5.5\std{0.6} & 17.6\std{0.8} & 26.1\std{0.6} & 12.6\std{0.6} & 6.8\std{2.9} & 21.8\std{8.4} & 32.4\std{11.4} & 15.2\std{5.4}\\
 & & MMS & 16.0\std{0.8} & 44.5\std{0.4} & 58.5\std{0.7} & 29.5\std{0.5} & 8.3\std{0.6} & 24.6\std{0.9} & 35.7\std{0.9} & 17.2\std{0.6} & 7.5\std{0.2} & 22.2\std{0.5} & 33.0\std{0.9} & 15.8\std{0.4} & 9.6\std{0.8} & 26.9\std{1.1} & 38.5\std{1.5} & 18.9\std{0.9} & 10.4\std{3.9} & 29.6\std{10.1} & 41.4\std{11.6} & 20.4\std{6.2}\\
 & & AMM & 20.0\std{0.7} & 51.5\std{1.0} & 66.5\std{1.2} & 34.8\std{0.4} & 9.1\std{0.5} & 27.1\std{0.7} & 38.8\std{0.9} & 18.6\std{0.5} & 8.9\std{0.6} & 26.6\std{0.7} & 38.5\std{1.5} & 18.4\std{0.7} & 10.6\std{0.6} & 29.5\std{0.9} & 41.4\std{0.9} & 20.6\std{0.6} & 12.1\std{5.3} & 33.7\std{12.0} & 46.3\std{13.5} & 23.1\std{7.9}\\
\cline{2-23}
 & \multirow{4}{*}{bert}
 & NCE & 38.2\std{1.2} & 71.6\std{1.0} & 82.2\std{0.8} & 53.0\std{1.0} & 11.8\std{0.7} & 33.2\std{0.7} & 45.0\std{0.7} & 22.6\std{0.4} & 19.3\std{1.0} & 43.8\std{0.7} & 57.4\std{1.3} & 31.3\std{0.9} & 13.0\std{1.0} & 33.9\std{1.8} & 45.8\std{1.9} & 23.5\std{1.3} & 20.6\std{12.2} & 45.6\std{18.0} & 57.6\std{17.4} & 32.6\std{14.1}\\
 & & SHN & 28.3\std{0.8} & 61.3\std{0.7} & 74.7\std{1.2} & 43.4\std{0.8} & 8.7\std{0.4} & 27.1\std{0.5} & 39.2\std{1.1} & 18.5\std{0.5} & 12.2\std{0.6} & 32.9\std{0.9} & 45.2\std{0.8} & 22.9\std{0.7} & 9.0\std{1.0} & 26.2\std{1.6} & 37.7\std{1.5} & 18.4\std{1.1} & 14.6\std{9.3} & 36.9\std{16.6} & 49.2\std{17.3} & 25.8\std{11.9}\\
 & & MMS & 35.9\std{0.5} & 70.1\std{0.7} & 81.6\std{1.0} & 51.0\std{0.3} & 11.6\std{0.7} & 32.4\std{0.3} & 44.7\std{1.0} & 22.2\std{0.3} & 17.2\std{0.5} & 42.2\std{0.9} & 55.8\std{1.4} & 29.6\std{0.6} & 12.2\std{0.9} & 32.4\std{2.5} & 44.1\std{2.2} & 22.5\std{1.4} & 19.2\std{11.4} & 44.3\std{17.8} & 56.6\std{17.5} & 31.3\std{13.6}\\
 & & AMM & 37.8\std{1.7} & 72.6\std{1.0} & 83.1\std{0.7} & 53.1\std{1.3} & 11.5\std{0.3} & 32.6\std{0.5} & 44.6\std{0.5} & 22.0\std{0.3} & 17.5\std{0.7} & 42.6\std{0.8} & 55.3\std{0.9} & 29.7\std{0.7} & 11.8\std{0.8} & 32.2\std{1.9} & 43.8\std{1.7} & 22.2\std{1.2} & 19.7\std{12.4} & 45.0\std{19.0} & 56.7\std{18.4} & 31.8\std{14.7}\\
\cline{2-23}
 & \multirow{4}{*}{bart}
 & NCE & 41.5\std{1.2} & 75.8\std{1.1} & 85.6\std{1.1} & 56.5\std{1.0} & 13.7\std{0.4} & 36.9\std{0.6} & 49.6\std{0.8} & 25.2\std{0.2} & 20.9\std{1.0} & 46.6\std{1.0} & 59.3\std{1.5} & 33.4\std{0.8} & 13.4\std{1.0} & 35.4\std{1.5} & 48.1\std{2.1} & 24.4\std{1.1} & 22.4\std{13.2} & 48.7\std{18.8} & 60.7\std{17.4} & 34.9\std{15.0}\\
 & & SHN & 21.3\std{0.9} & 52.1\std{0.8} & 66.3\std{0.8} & 35.7\std{0.7} & 7.1\std{0.4} & 22.1\std{0.7} & 33.2\std{0.9} & 15.5\std{0.4} & 10.9\std{0.4} & 30.5\std{1.4} & 41.9\std{1.3} & 21.1\std{0.7} & 7.7\std{0.7} & 24.4\std{1.0} & 34.9\std{1.1} & 16.7\std{0.9} & 11.8\std{6.6} & 32.3\std{13.7} & 44.1\std{15.3} & 22.2\std{9.3}\\
 & & MMS & 44.1\std{1.1} & 78.7\std{0.7} & 87.4\std{0.5} & 59.1\std{0.7} & 14.5\std{0.5} & 38.0\std{0.6} & 50.9\std{0.9} & 25.9\std{0.3} & 23.1\std{0.7} & 49.3\std{1.2} & 61.7\std{1.6} & 35.7\std{0.8} & 14.5\std{1.1} & 36.3\std{1.2} & 49.5\std{1.8} & 25.6\std{1.1} & 24.0\std{14.0} & 50.6\std{19.6} & 62.4\std{17.6} & 36.6\std{15.7}\\
 & & AMM & \textbf{45.3}\std{0.5} & \textbf{80.0}\std{0.5} & \textbf{87.6}\std{0.8} & \textbf{60.3}\std{0.4} & 15.2\std{0.5} & 39.1\std{0.7} & 51.4\std{0.9} & 26.7\std{0.5} & 21.9\std{1.0} & 49.2\std{1.6} & 61.8\std{1.4} & 34.9\std{1.1} & 15.0\std{1.4} & 37.0\std{1.8} & 48.7\std{1.9} & 25.9\std{1.5} & 24.4\std{14.3} & 51.3\std{19.8} & 62.4\std{17.7} & 37.0\std{16.1}\\
\hline
\multirow{12}{*}{\textbf{ActivityNet}} & \multirow{4}{*}{fasttext}
 & NCE & 13.6\std{0.6} & 38.0\std{1.0} & 50.4\std{0.9} & 25.6\std{0.7} & 12.5\std{1.0} & 36.4\std{1.1} & 50.8\std{0.7} & 24.5\std{0.7} & 9.5\std{0.6} & 26.8\std{1.2} & 38.9\std{1.2} & 18.9\std{0.6} & 7.9\std{1.1} & 25.1\std{1.4} & 36.6\std{1.2} & 17.3\std{1.1} & 10.9\std{2.6} & 31.6\std{6.6} & 44.2\std{7.5} & 21.6\std{4.1}\\
 & & SHN & 13.0\std{0.7} & 37.2\std{0.8} & 50.2\std{1.2} & 24.8\std{0.9} & 10.9\std{0.7} & 32.2\std{0.4} & 45.7\std{0.6} & 21.8\std{0.4} & 8.8\std{0.8} & 24.4\std{1.4} & 35.6\std{0.8} & 17.6\std{0.8} & 6.7\std{0.6} & 21.5\std{0.8} & 31.4\std{0.8} & 14.9\std{0.6} & 9.9\std{2.7} & 28.8\std{7.2} & 40.7\std{8.7} & 19.8\std{4.4}\\
 & & MMS & 14.2\std{0.4} & 39.1\std{0.7} & 52.8\std{0.8} & 26.5\std{0.4} & 12.7\std{0.2} & 37.1\std{0.9} & 50.5\std{0.5} & 24.5\std{0.5} & 8.8\std{0.6} & 25.8\std{0.5} & 37.5\std{0.7} & 18.0\std{0.5} & 7.9\std{0.5} & 23.3\std{1.0} & 34.0\std{0.6} & 16.4\std{0.5} & 10.9\std{3.0} & 31.3\std{7.9} & 43.7\std{9.3} & 21.4\std{4.9}\\
 & & AMM & 13.0\std{0.8} & 36.8\std{0.4} & 49.4\std{0.3} & 24.6\std{0.6} & 12.7\std{0.4} & 37.2\std{0.4} & 51.0\std{0.8} & 24.8\std{0.4} & 8.8\std{0.8} & 25.5\std{0.9} & 36.1\std{1.2} & 17.7\std{0.8} & 8.1\std{0.8} & 24.4\std{1.1} & 35.4\std{1.3} & 17.0\std{0.9} & 10.6\std{2.6} & 31.0\std{7.0} & 43.0\std{8.4} & 21.0\std{4.3}\\
\cline{2-23}
 & \multirow{4}{*}{bert}
 & NCE & 19.0\std{1.1} & 48.1\std{0.7} & 62.3\std{0.8} & 32.8\std{0.9} & 14.8\std{0.9} & 41.0\std{0.7} & 54.6\std{1.1} & 27.4\std{0.9} & 13.1\std{1.1} & 33.7\std{1.2} & 46.8\std{0.9} & 23.8\std{1.1} & 7.4\std{0.7} & 22.8\std{1.2} & 34.1\std{1.5} & 16.0\std{0.7} & 13.6\std{4.8} & 36.4\std{10.8} & 49.4\std{12.0} & 25.0\std{7.0}\\
 & & SHN & 17.1\std{0.5} & 44.4\std{0.5} & 58.6\std{0.5} & 30.2\std{0.3} & 12.4\std{0.8} & 35.8\std{0.8} & 49.2\std{0.4} & 24.2\std{0.6} & 9.2\std{0.2} & 26.8\std{0.8} & 37.8\std{1.2} & 18.7\std{0.5} & 6.2\std{0.3} & 20.1\std{0.9} & 30.1\std{1.6} & 14.1\std{0.4} & 11.2\std{4.7} & 31.8\std{10.6} & 43.9\std{12.5} & 21.8\std{7.0}\\
 & & MMS & 19.4\std{1.0} & 48.1\std{1.2} & 62.4\std{1.2} & 33.0\std{0.9} & 14.2\std{1.3} & 39.6\std{1.0} & 52.5\std{1.0} & 26.6\std{1.2} & 12.8\std{1.1} & 33.6\std{1.1} & 45.5\std{0.9} & 23.5\std{1.0} & 7.4\std{0.7} & 22.2\std{0.7} & 32.8\std{0.7} & 15.8\std{0.7} & 13.4\std{4.9} & 35.9\std{10.9} & 48.3\std{12.4} & 24.7\std{7.1}\\
 & & AMM & 20.5\std{1.1} & 48.7\std{0.9} & 62.4\std{0.8} & 33.9\std{0.7} & 15.1\std{1.3} & 40.8\std{1.0} & 53.9\std{0.6} & 27.5\std{1.1} & 12.7\std{0.4} & 33.4\std{0.6} & 45.1\std{0.9} & 23.5\std{0.4} & 7.3\std{0.7} & 21.9\std{1.4} & 32.0\std{1.5} & 15.4\std{0.9} & 13.9\std{5.5} & 36.2\std{11.4} & 48.3\std{13.0} & 25.1\std{7.7}\\
\cline{2-23}
 & \multirow{4}{*}{bart}
 & NCE & 25.3\std{0.7} & 57.7\std{0.9} & 70.8\std{0.9} & 40.1\std{0.5} & 14.3\std{0.6} & 39.2\std{0.8} & 53.8\std{1.0} & 26.7\std{0.5} & 14.9\std{0.6} & 37.3\std{1.3} & 50.8\std{1.6} & 26.4\std{0.7} & 9.7\std{1.0} & 28.5\std{1.2} & 41.1\std{1.0} & 19.8\std{1.0} & 16.0\std{6.6} & 40.7\std{12.3} & 54.1\std{12.4} & 28.2\std{8.5}\\
 & & SHN & 21.6\std{1.1} & 51.9\std{0.8} & 66.2\std{0.6} & 35.7\std{0.9} & 11.8\std{0.9} & 34.9\std{0.8} & 49.3\std{0.7} & 23.4\std{0.9} & 12.8\std{0.7} & 31.9\std{0.7} & 44.5\std{1.6} & 23.0\std{0.6} & 7.9\std{1.0} & 24.5\std{0.9} & 35.1\std{1.4} & 16.8\std{1.0} & 13.5\std{5.8} & 35.8\std{11.6} & 48.8\std{13.0} & 24.7\std{7.9}\\
 & & MMS & 26.1\std{0.9} & 58.3\std{0.8} & 70.9\std{0.7} & 40.7\std{0.5} & 14.1\std{0.4} & 39.0\std{0.2} & 52.8\std{1.2} & 26.4\std{0.2} & 15.9\std{0.7} & 39.1\std{1.0} & 52.0\std{1.4} & 27.5\std{0.7} & 10.2\std{0.6} & 29.1\std{0.8} & 41.3\std{1.1} & 20.1\std{0.7} & 16.6\std{6.8} & 41.4\std{12.2} & 54.2\std{12.3} & 28.7\std{8.7}\\
 & & AMM & 25.0\std{1.3} & 56.0\std{1.0} & 68.4\std{0.6} & 39.1\std{1.1} & \textbf{19.1}\std{1.0} & \textbf{48.1}\std{1.2} & \textbf{61.2}\std{0.6} & \textbf{32.5}\std{0.6} & 15.1\std{0.9} & 37.1\std{1.4} & 50.4\std{1.5} & 26.4\std{0.9} & 9.4\std{1.1} & 26.2\std{1.5} & 37.1\std{1.4} & 18.3\std{1.2} & 17.1\std{6.6} & 41.8\std{13.0} & 54.3\std{13.6} & 29.1\std{8.9}\\
\hline
\multirow{12}{*}{\textbf{MSR-VTT}} & \multirow{4}{*}{fasttext}
 & NCE & 9.1\std{0.3} & 27.2\std{0.4} & 39.1\std{0.5} & 18.6\std{0.2} & 5.7\std{0.5} & 17.8\std{0.7} & 27.0\std{0.8} & 12.8\std{0.4} & 11.5\std{0.6} & 34.5\std{1.4} & 49.4\std{1.4} & 23.3\std{0.7} & 7.7\std{0.6} & 24.2\std{0.9} & 35.5\std{1.7} & 16.7\std{0.9} & 8.5\std{2.4} & 25.9\std{6.9} & 37.8\std{9.3} & 17.9\std{4.4}\\
 & & SHN & 6.5\std{0.3} & 20.8\std{0.7} & 31.5\std{1.0} & 14.6\std{0.3} & 4.4\std{0.4} & 14.0\std{0.6} & 21.7\std{0.3} & 10.4\std{0.4} & 8.9\std{0.4} & 28.4\std{0.8} & 41.4\std{0.6} & 19.2\std{0.4} & 5.9\std{0.5} & 17.9\std{1.0} & 26.3\std{1.2} & 12.7\std{0.6} & 6.4\std{1.9} & 20.3\std{6.1} & 30.2\std{8.5} & 14.2\std{3.7}\\
 & & MMS & 7.5\std{0.3} & 24.4\std{1.0} & 36.3\std{1.2} & 16.7\std{0.5} & 5.0\std{0.3} & 17.3\std{0.5} & 26.5\std{0.8} & 12.2\std{0.2} & 10.5\std{0.5} & 31.7\std{0.5} & 44.8\std{0.9} & 21.5\std{0.5} & 7.3\std{0.3} & 21.7\std{1.4} & 32.8\std{1.5} & 15.6\std{0.4} & 7.6\std{2.3} & 23.8\std{6.0} & 35.1\std{7.6} & 16.5\std{3.8}\\
 & & AMM & 11.4\std{0.7} & 33.0\std{1.0} & 46.3\std{0.6} & 22.4\std{0.6} & 6.0\std{0.5} & 20.2\std{0.5} & 29.9\std{0.5} & 13.8\std{0.3} & 16.3\std{0.4} & 43.1\std{0.5} & 57.4\std{1.1} & 29.1\std{0.4} & 8.4\std{0.2} & 25.5\std{1.0} & 37.1\std{1.3} & 17.5\std{0.4} & 10.5\std{4.4} & 30.5\std{9.9} & 42.7\std{11.9} & 20.7\std{6.6}\\
\cline{2-23}
 & \multirow{4}{*}{bert}
 & NCE & 16.2\std{0.7} & 42.3\std{0.7} & 56.1\std{0.8} & 28.9\std{0.4} & 5.6\std{0.6} & 18.8\std{0.9} & 29.0\std{0.8} & 13.2\std{0.5} & 20.9\std{0.6} & 52.4\std{0.9} & 67.8\std{1.4} & 35.8\std{0.6} & 8.1\std{0.8} & 24.6\std{1.6} & 36.5\std{1.0} & 17.3\std{0.9} & 12.7\std{7.1} & 34.5\std{15.6} & 47.3\std{17.8} & 23.8\std{10.4}\\
 & & SHN & 9.2\std{0.3} & 26.9\std{0.5} & 39.0\std{0.4} & 18.8\std{0.4} & 4.6\std{0.2} & 16.2\std{0.6} & 25.5\std{0.6} & 11.5\std{0.2} & 12.8\std{0.2} & 35.9\std{0.6} & 48.9\std{0.4} & 24.3\std{0.2} & 5.3\std{0.7} & 17.2\std{1.3} & 27.1\std{0.7} & 12.5\std{0.9} & 8.0\std{3.8} & 24.0\std{9.3} & 35.1\std{11.0} & 16.8\std{6.0}\\
 & & MMS & 16.9\std{0.7} & 42.6\std{0.4} & 55.9\std{1.0} & 29.5\std{0.5} & 5.9\std{0.4} & 19.2\std{0.8} & 29.2\std{0.5} & 13.6\std{0.5} & 22.8\std{0.7} & 56.1\std{0.9} & 71.2\std{1.1} & 38.2\std{0.6} & 8.1\std{0.9} & 24.8\std{1.9} & 36.3\std{2.0} & 17.3\std{1.2} & 13.4\std{7.9} & 35.7\std{16.9} & 48.2\std{19.1} & 24.7\std{11.3}\\
 & & AMM & 14.6\std{0.3} & 38.8\std{1.1} & 52.3\std{0.8} & 26.6\std{0.4} & 6.2\std{0.9} & 20.3\std{1.3} & 30.2\std{1.2} & 14.1\std{0.9} & 25.8\std{1.1} & 59.5\std{1.0} & 73.9\std{1.3} & 41.0\std{1.0} & 8.2\std{0.6} & 23.4\std{1.2} & 33.5\std{1.2} & 16.6\std{0.7} & 13.7\std{8.8} & 35.5\std{17.9} & 47.5\std{20.1} & 24.6\std{12.2}\\
\cline{2-23}
 & \multirow{4}{*}{bart}
 & NCE & 18.2\std{0.5} & 45.7\std{1.0} & 59.9\std{1.3} & 31.4\std{0.5} & 7.5\std{0.4} & 22.8\std{1.3} & 33.8\std{1.1} & 15.9\std{0.7} & 23.8\std{1.2} & 54.5\std{0.9} & 69.1\std{0.9} & 38.2\std{1.0} & 9.5\std{0.6} & 27.6\std{1.6} & 39.0\std{1.6} & 19.1\std{0.9} & 14.8\std{7.6} & 37.7\std{14.9} & 50.4\std{16.8} & 26.1\std{10.4}\\
 & & SHN & 11.4\std{0.6} & 30.6\std{0.3} & 42.5\std{0.7} & 21.4\std{0.5} & 5.4\std{0.7} & 17.6\std{0.7} & 27.1\std{0.4} & 12.6\std{0.7} & 14.6\std{0.9} & 39.5\std{0.7} & 53.1\std{1.1} & 26.9\std{0.8} & 6.0\std{0.7} & 19.0\std{1.2} & 28.8\std{1.6} & 13.6\std{0.9} & 9.4\std{4.4} & 26.7\std{10.3} & 37.9\std{12.3} & 18.6\std{6.8}\\
 & & MMS & 16.7\std{0.6} & 41.6\std{0.8} & 55.2\std{0.7} & 29.1\std{0.5} & 7.2\std{0.7} & 23.6\std{1.3} & 34.7\std{1.0} & 16.1\std{0.8} & 23.0\std{0.9} & 54.8\std{0.6} & 68.9\std{0.7} & 37.6\std{0.6} & 8.7\std{0.7} & 26.0\std{1.4} & 37.3\std{1.1} & 18.0\std{0.8} & 13.9\std{7.4} & 36.5\std{14.6} & 49.0\std{16.1} & 25.2\std{10.1}\\
 & & AMM & 16.6\std{0.8} & 42.2\std{0.8} & 55.7\std{1.1} & 29.1\std{0.6} & 8.0\std{0.6} & 23.7\std{1.5} & 34.7\std{1.5} & 16.6\std{0.8} & 24.0\std{0.7} & 57.4\std{0.9} & 72.1\std{1.1} & 39.2\std{0.5} & 9.1\std{0.7} & 26.7\std{1.2} & 39.1\std{1.7} & 18.7\std{0.8} & 14.4\std{7.4} & 37.5\std{15.5} & 50.4\std{17.1} & 25.9\std{10.4}\\
\hline
\multirow{12}{*}{\textbf{S-MiT}} & \multirow{4}{*}{fasttext}
 & NCE & 15.5\std{0.6} & 41.5\std{0.7} & 54.3\std{0.6} & 28.0\std{0.5} & 9.0\std{0.4} & 26.7\std{0.8} & 38.5\std{0.8} & 18.5\std{0.4} & 10.1\std{0.7} & 28.8\std{0.6} & 39.9\std{0.4} & 19.7\std{0.5} & \\
 & & SHN & 13.9\std{0.6} & 38.2\std{0.8} & 50.4\std{1.0} & 25.8\std{0.3} & 8.7\std{0.4} & 26.1\std{0.7} & 36.9\std{0.6} & 18.0\std{0.2} & 8.9\std{0.6} & 23.8\std{0.4} & 35.0\std{1.3} & 17.4\std{0.4} & \\
 & & MMS & 14.6\std{1.0} & 39.0\std{1.2} & 52.7\std{1.5} & 26.7\std{1.0} & 8.9\std{0.6} & 26.9\std{0.5} & 37.9\std{0.5} & 18.4\std{0.4} & 9.3\std{0.6} & 26.3\std{0.6} & 37.4\std{0.6} & 18.6\std{0.5} & \\
 & & AMM & 13.8\std{0.8} & 37.3\std{1.4} & 49.3\std{1.3} & 25.3\std{0.7} & 10.6\std{0.3} & 30.1\std{0.6} & 41.7\std{0.4} & 20.7\std{0.2} & 9.9\std{0.2} & 27.9\std{0.7} & 38.7\std{0.7} & 19.3\std{0.2} & \\
\cline{2-23}
 & \multirow{4}{*}{bert}
 & NCE & 37.3\std{0.7} & 69.9\std{1.1} & 81.0\std{1.2} & 51.9\std{0.7} & 12.0\std{0.4} & 33.0\std{1.0} & 45.0\std{1.0} & 22.7\std{0.3} & 28.3\std{0.7} & 59.3\std{1.0} & 73.2\std{0.6} & 42.7\std{0.7} & 26.6\std{1.6} & 56.5\std{1.6} & 69.3\std{1.6} & 40.5\std{1.5} & 26.0\std{10.5} & 54.7\std{15.6} & 67.1\std{15.5} & 39.5\std{12.2}\\
 & & SHN & 29.6\std{0.4} & 60.8\std{0.2} & 72.8\std{0.7} & 43.9\std{0.5} & 9.6\std{0.5} & 27.3\std{0.8} & 38.2\std{1.1} & 18.9\std{0.4} & 19.7\std{1.0} & 45.6\std{0.9} & 58.7\std{0.7} & 32.3\std{0.9} & 21.1\std{0.8} & 47.8\std{1.4} & 61.1\std{1.3} & 33.9\std{0.9} & 20.0\std{8.2} & 45.4\std{13.8} & 57.7\std{14.4} & 32.2\std{10.3}\\
 & & MMS & 36.0\std{1.0} & 68.5\std{1.2} & 79.5\std{1.2} & 50.5\std{0.9} & 12.2\std{0.7} & 33.0\std{0.7} & 44.9\std{1.1} & 22.8\std{0.7} & 27.8\std{0.9} & 59.0\std{0.6} & 72.1\std{1.3} & 42.1\std{0.8} & 27.2\std{1.7} & 57.1\std{1.4} & 69.7\std{1.4} & 41.0\std{1.5} & 25.8\std{9.9} & 54.4\std{15.1} & 66.6\std{15.0} & 39.1\std{11.7}\\
 & & AMM & 36.6\std{0.7} & 69.3\std{1.0} & 79.8\std{0.9} & 51.2\std{0.7} & 13.4\std{0.7} & 34.1\std{0.6} & 45.6\std{0.3} & 23.6\std{0.5} & 27.9\std{1.1} & 58.6\std{0.6} & 71.0\std{0.5} & 42.0\std{0.9} & 30.6\std{1.7} & 59.2\std{1.7} & 70.0\std{1.7} & 43.8\std{1.6} & 27.1\std{9.8} & 55.3\std{15.0} & 66.6\std{14.7} & 40.2\std{11.7}\\
\cline{2-23}
 & \multirow{4}{*}{bart}
 & NCE & 42.4\std{0.5} & 74.4\std{1.3} & 84.0\std{1.3} & 56.7\std{0.7} & 15.4\std{0.5} & 38.2\std{1.2} & 50.4\std{1.0} & 26.7\std{0.8} & 31.2\std{0.8} & 62.0\std{0.7} & 74.1\std{0.7} & 45.2\std{0.6} & \\
 & & SHN & 38.7\std{0.7} & 72.3\std{1.3} & 82.2\std{1.1} & 53.5\std{0.7} & 13.2\std{0.7} & 33.4\std{1.0} & 45.3\std{0.7} & 23.5\std{0.5} & 27.1\std{1.1} & 57.3\std{1.1} & 69.7\std{0.8} & 41.0\std{0.9} & \\
 & & MMS & 39.9\std{0.6} & 72.9\std{1.0} & 82.6\std{0.7} & 54.5\std{0.4} & 15.2\std{0.7} & 37.3\std{0.2} & 49.6\std{0.5} & 26.3\std{0.6} & 29.4\std{1.1} & 58.7\std{0.8} & 70.8\std{0.7} & 43.1\std{0.9} & \\
 & & AMM & 42.7 & 75.4 & 84.2 & 57.1 & 17.6 & 41.6 & 53.8 & 29.2 & \textbf{33.1} & \textbf{64.8} & \textbf{77.4} & \textbf{47.6} & \textbf{34.8} & \textbf{64.4} & \textbf{75.1} & \textbf{48.3} & \textbf{32.1} & \textbf{57.3} & \textbf{77.8} & \textbf{45.6}\\
\hline
    \end{tabular}}
\caption{\textbf{Cross Dataset Evaluation on Video/Caption Retrieval:} Here we compare the generalization performance of models trained on four different datasets for video/caption retrieval.  Each model is trained on a single dataset and evaluated on the test set from each other dataset.  We additionally show the mean performance across datasets.}
\label{table:full_cross_evaluation}
\end{table*}

\begin{table*}
    \scalebox{0.62}{
    \begin{tabular}{ c | c  c  c  c | c  c  c  c | c  c  c  c }
        \Xhline{0.8pt}
        \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{4}{c|}{\textbf{Caption to Video}} & \multicolumn{4}{c|}{\textbf{Video to Caption}} & \multicolumn{4}{c}{\textbf{Mean}} \\
         & R@1 & R@5 & R@10 & mAP & R@1 & R@5 & R@10 & mAP & R@1 & R@5 & R@10 & mAP \\
        \Xhline{0.8pt}
        \multirow{5}{*}{Vatex \cite{Wang_2019_ICCV}}
        & 11.8 & 33.6 & 47.2 & 22.8 & 13.4 & 37.4 & 50.6 & 25.3 & 12.6 & 35.5 & 48.9 & 24.1\\
        \hline
        \multirow{5}{*}{ActivityNet \cite{krishna2017dense}}
        & \\
        \hline
        \multirow{5}{*}{MSR-VTT \cite{xu2016msr-vtt}}
        & \\
        \hline
        \multirow{5}{*}{S-MiT}
        & \\
        \Xhline{0.8pt}
    \end{tabular}}
\caption{\textbf{Loss Function Comparison for Video/Caption Retrieval on Full Test Set:}  Models trained on four datasets evaluated for video/caption retrieval on their full test sets.}
\label{table:loss_comparison}

\section{Video/Caption Retrieval}

Table~\ref{table:full_loss_comparison_language} shows results on using different combinations of the loss functions and language models on {Vatex}~\cite{Wang_2019_ICCV}, {ActivityNet Captions}~\cite{krishna2017dense}, {MSR-VTT}~\cite{xu2016msr-vtt} as well as the proposed Spoken Moments. 

In Table~\ref{table:full_cross_evaluation}, we also extend the cross-dataset evaluation shown in Table 6 by using models trained with the different loss functions, language models, and datasets from Table~\ref{table:full_loss_comparison_language}.  Results are slightly different here than in Table 6 as we perform this analysis by only training the projection layers and not the visual base model (TSM+2D).  For both tables, the results are averaged over five rounds with a single random batch of 1k caption-video pairs from the test set of the specified dataset.\footnote{For evaluation, we use the public test set for Vatex, the second validation set for ActivityNet Captions, and the test set for MSR-VTT.}


